Efficient reconstruction, benchmarking and validation of cross-talk models in readout noise in near-term quantum devices

Readout errors contribute significantly to the overall noise affecting present-day quantum computers. However, the complete characterization of generic readout noise is infeasible for devices consisting of a large number of qubits. Here we introduce an appropriately tailored quantum detector tomography protocol, the so called Quantum Detector Overlapping Tomography, which enables efficient characterization of $k-$local cross-talk effects in the readout noise as the sample complexity of the protocol scales logarithmically with the total number of qubits. We show that QDOT data provides information about suitably defined reduced POVM operators, correlations and coherences in the readout noise, as well as allows to reconstruct the correlated clusters and neighbours readout noise model. Benchmarks are introduced to verify utility and accuracy of the reconstructed model. We apply our method to investigate cross-talk effects on 79 qubit Rigetti and 127 qubit IBM devices. We discuss their readout noise characteristics, and demonstrate effectiveness of our approach by showing superior performance of correlated clusters and neighbours over models without cross-talk in model-based readout error mitigation applied to energy estimation of MAX-2-SAT Hamiltonians, with the improvement on the order of 20% for both devices.

==> sections/coherence_indicator.tex <==
\section{Lower bound on Coherence strength}
\label{sec:CS_lower_bound}
In this section a lower bound on coherence strength of noisy POVM $\M$ is proved. 
\begin{prop}
For a POVM $\M$ and quantum states $|p\rangle, |q\rangle$ constructed from tensor product of Pauli $X,Y$ eigenstates the following bound holds 
\begin{eqnarray}
    \mathrm{CS}(\M)^{AC} \geq \frac{\tvd \left( \Pr(p), \Pr(q)   \right)}{d \| \delta_{p,q} \|_{HS}},
\end{eqnarray}
where $\Pr(p)$ ($\Pr(q)$) is probability distribution obtained by measuring $|p\rangle$ ($|q\rangle$)  with $\M$, and $\delta_{p,q} =  \left( | p \rangle \langle p | - | q \rangle \langle q | \right ) $, and $d$ is  dimension of the corresponding Hilbert space. 

\end{prop}

\begin{proof}
Let us decompose effects of $\M$ into diagonal and off-diagonal part $M_i =M_i^{diag} + \Delta_i$. For a particular outcome $i$ it holds

\begin{eqnarray}
    &&\Pr(i|p) - \Pr(i|q) = \tr \left( M_i \left( | p \rangle \langle p | - | q \rangle \langle q | \right) \right) = \tr \left( \Delta_i \left( | p \rangle \langle p | - | q \rangle \langle q | \right ) \right) =\tr \left( \Delta_i \delta_{p,q} \right) \leq \| \Delta_i \|_{HS} \| \delta_{p,q} \|_{HS},
\end{eqnarray}
where the second equality follows from the fact that the states $| p \rangle \langle p |, | q \rangle \langle q |$ differ only on off-diagonal elements. Using this fact we can write 

\begin{eqnarray}
     &&\tvd \left( \Pr(p), \Pr(q)   \right) \leq \frac{1}{2} \sum_i \sqrt{ \| \Delta_i \|_{HS}^2} \sqrt{\| \delta_{p,q} \|^2_{HS}} \leq \frac{1}{2}  \| \delta_{p,q} |_{HS} \sum_i  \sqrt{  \| \Delta_{i} |^2_{HS} + \tr \left( \Delta_{i}  \right)^2} \leq \\ 
    && d \times \| \delta_{p,q} |_{HS} \times  \dist_{AV} (\M, \Phi_{\text{dep}}(\M) ),
\end{eqnarray}
where the last inequality follows from the definition of average case distance. By using definition of coherence strength $\mathrm{CS}(\M)^{AC}$  the bound is obtained. 






\end{proof}

\begin{prop}
Consider $\hat{\mathrm{CS}}(\M)^{AC}$ that is an empirical estimation of $\mathrm{CS}(\M)^{AC}$. It holds that
\begin{eqnarray}
\label{eq:cs_experimental}
  \left|   \mathrm{CS}(\M)^{AC} -  \hat{\mathrm{CS}}(\M)^{AC}  \right| \leq  \frac{\epsilon_{p}+ \epsilon_{q}}{d}.
\end{eqnarray}
where  $\epsilon_{p}$, $\epsilon_{q}$ are upper bounds on distances between true distributions $\Pr(p), \Pr(q)$, and their empirical values $\hat{\Pr}(p), \hat{\Pr}(q)$.        
\end{prop}
\begin{proof}
From the fact that $\tvd \left( \Pr(p), \hat{\Pr}(p)   \right) \leq \epsilon_{p}$, and  $\tvd \left( \Pr(q),  \hat{\Pr}(q) \right) \leq \epsilon_{q}$ it follows that
\begin{eqnarray}
    && \left| \tvd \left( \Pr(p), \Pr(q)   \right) - \tvd \left( \hat{\Pr}(p), \hat{\Pr}(q)   \right) \right|    \leq \epsilon_{p} + \epsilon_{q}. 
\end{eqnarray}
From the above inequality one obtains the bound (\ref{eq:cs_experimental}).
\end{proof}

The probabilistic upper bounds on $\epsilon_{p}, \epsilon_{q}$ are obtained using the results of \cite{Weissman2003}:

\begin{eqnarray}
       \tvd\left( \Pr(p), \hat{\Pr}(p)   \right) \leq \epsilon^*_{p}= \sqrt{\frac{\log\rbracket{2^d-2}-\log{\rbracket{P_{ \text{err}}}}}{2 N_S}} ,
\end{eqnarray}
where $N_S$ is the number of shots used in the estimation, and  $P_{ \text{err}}$ denotes the error probability:  $\text{Pr}\rbracket{\tvd \left( \Pr(p), \hat{\Pr}(p)   \right) \geq \epsilon_p}$.
%    

